Decoupled execution of synchronous coordination models via behavioural automata

Synchronous coordination systems allow the exchange of data by logically indivisible actions involving all coordinated entities. This paper introduces behavioural automata, a logically synchronous coordination model based on the Reo coordination language, which focuses on relevant aspects for the concurrent evolution of these systems. We show how our automata model encodes the Reo and Linda coordination models and how it introduces an explicit predicate that captures the concurrent evolution, distinguishing local from global actions, and lifting the need of most synchronous models to involve all entities at each coordination step, paving the way to more scalable implementations.

==> eptcsdata.tex <==
\providecommand{\firstpage}{65}
\providecommand{\publicationstatus}{M.R. Mousavi and A. Ravara: FOCLASA 2011\\
EPTCS 58, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.58.5}{10.4204/EPTCS.58.5}}
\pdfoutput=1

